NorQuAD: Norwegian Question Answering Dataset

In this paper we present NorQuAD: the first Norwegian question answering dataset for machine reading comprehension. The dataset consists of 4,752 manually created question-answer pairs. We here detail the data collection procedure and present statistics of the dataset. We also benchmark several multilingual and Norwegian monolingual language models on the dataset and compare them against human performance. The dataset will be made freely available.

==> NoDaLiDa2023-NorQuAD-paper copy/plots/beginningendplot.tex <==
\begin{figure}
    \centering

    \begin{tikzpicture}
        \begin{axis}[
            symbolic x coords={Beginning, End},
            xtick={Beginning, End},
            legend style={at={(0.96,0.23)},anchor=east},
            ymin=50,
        ]
        
        \addplot coordinates {
                                        (Beginning,84.99)
                                        (End,91.83)
                };
        \addplot coordinates {
                                        (Beginning,92.84)
                                        (End,94.37)
                };
        \addplot+[ error bars/.cd,
                        y dir=both,
                        y explicit
                    ] coordinates {
                                        (Beginning,67.67) +- (0,1.5)
                                        (End,80.35) +- (0,1.5)
                };
        \addplot+[ error bars/.cd,
                        y dir=both,
                        y explicit
                    ] coordinates {
                                        (Beginning,80.06) +- (0,1.5)
                                        (End,80.36) +- (0,1.5)
                };
        \legend{Human Wiki, Human news, NB-BERT Wiki, NB-BERT news}
        \end{axis}
    \end{tikzpicture}
    \caption{Performance on the beginning and end of datasets (F1 score)}
    \label{fig:beginningend}
\end{figure}


==> NoDaLiDa2023-NorQuAD-paper copy/plots/performanceplot.tex <==
\begin{figure*}
    \centering
    \resizebox{.65\textwidth}{!}{
    \begin{tikzpicture}
        \begin{axis}[
            xbar,
            xmax=97,
            y = 35pt,
            % Change order in symbolic y coords:
            symbolic y coords={mBERT,NorBERT2,XLM-RoBERTa,NB-BERT$_{ger}$,NB-BERT,Human},
            ytick={NorBERT2,NB-BERT,mBERT,XLM-RoBERTa,NB-BERT$_{ger}$,Human},
            nodes near coords, nodes near coords align={horizontal},
            every node near coord/.append style={yshift=0.4cm, xshift=-0.4cm},
            axis x line*=bottom,
            label style={font=\tiny},
            legend style={at={(0.96,0.12)},anchor=east},
            reverse legend
            ]
        \addplot+[
                        error bars/.cd,
                        x dir=both,
                        x explicit
                    ]%[blue!20!black,fill=blue!80!white] 
                    coordinates {
                                (77.86,NorBERT2) +- (0.65,0)
                                (81.27,NB-BERT) +- (0.73,0)
                                (76.00,mBERT) +- (0.83,0)
                                (78.42,XLM-RoBERTa) +- (0.97,0)
                                (80.76,NB-BERT$_{ger}$) +- (0.62,0)
                                (91.14,Human)
        };
        \addplot+[
                        error bars/.cd,
                        x dir=both,
                        x explicit
                    ][red!20!black,fill=red!80!white] 
                    coordinates {
                                (64.64,NorBERT2) +- (1.40,0)
                                (69.68,NB-BERT) +- (1.21,0)
                                (63.32,mBERT) +- (1.58,0)
                                (64.52,XLM-RoBERTa) +- (1.37,0)
                                (68.78,NB-BERT$_{ger}$) +- (1.38,0)
                                (78.13,Human)
        };
        \legend{F1, EM}
        \end{axis}
    \end{tikzpicture}
    }
    \caption{Performance of annotators and models on the entire test set: EM and F1 scores}
    \label{fig:performance}
\end{figure*}

